Minimizers of the Willmore functional with a small area constraint

We show the existence of a smooth spherical surface minimizing the Willmore functional subject to an area constraint in a compact Riemannian three-manifold, provided the area is small enough. Moreover, we classify complete surfaces of Willmore type with positive mean curvature in Riemannian three-manifolds.

==> draft_commands.tex <==
\usepackage{ifthen}

%% Collect Time and Date Info
\makeatletter
\newcommand{\pt@twodigit}[1]{{\pt@tmp=#1\relax\ifnum\pt@tmp<10 0\fi\the\pt@tmp}}
\newcount\pt@hours
\newcount\pt@minutes
\newcount\pt@tmp
\newcommand{\printtime}{%
\pt@hours=\time%
\divide\pt@hours by 60\relax%
\pt@tmp=\pt@hours%
\multiply\pt@tmp by -60\relax%
\pt@minutes=\time%
\advance\pt@minutes by \pt@tmp%
\pt@twodigit\pt@hours:\pt@twodigit\pt@minutes}

%% How to put Info in the margin
\newlength{\mt@MarginWidth}
\newlength{\mt@PageHeight}
\newlength{\mt@ActualWidth}
\newlength{\mt@MaxWidth}
\newlength{\mt@FontSize}
\newlength{\mt@RightSkip}
\newlength{\mt@TextHeight}
\newlength{\mt@OffsetX}
\newlength{\mt@OffsetY}

\usepackage{eso-pic}
\usepackage{type1cm}
\usepackage{graphicx}

\newcommand{\margintext}[1]{
  \ifx\pdfoutput\undefined\write16{WARNING: Margintext
      will only correctly show up in PS - FILE!}
  \fi
  \AddToShipoutPicture{%
    \setlength{\mt@MarginWidth}{\oddsidemargin}%
    \addtolength{\mt@MarginWidth}{1in}%
    \setlength{\mt@PageHeight}{\paperheight}%
    \setlength{\mt@MaxWidth}{.8\mt@MarginWidth}%
    \setlength{\mt@FontSize}{12mm}%
    \setlength{\mt@RightSkip}{3mm}%
    \setlength{\mt@ActualWidth}{15mm}%
    \ifthenelse{\lengthtest{\mt@ActualWidth > \mt@MaxWidth}}%
    {
      \setlength{\mt@FontSize}{.6\mt@MarginWidth}
      \setlength{\mt@RightSkip}{.2\mt@MarginWidth}
      \setlength{\mt@ActualWidth}{.8\mt@MarginWidth}
    }{}
    \setlength{\mt@OffsetX}{\mt@ActualWidth}
    \setlength{\mt@OffsetY}{0mm}
    \setlength{\unitlength}{1pt}%
    \put(\strip@pt\mt@OffsetX,\strip@pt\mt@OffsetY){%
      \rotatebox{90}
        {
          \makebox[\mt@PageHeight][c]
          {\textcolor[gray]{0.75}{\fontfamily{cmss}
              \fontseries{m}
              \fontshape{n}
              \fontsize{\mt@FontSize}{\mt@FontSize}
              \selectfont{#1}}}
        }
      }
    }
}

%% Collect information from Subversion
% If the file svn_version.tex exists, we will read it, in there
% the command \svnVersion is defined. If the file does not exist, we
% print a warning and set \svnVersion to Unknown
\newboolean{draftmargin}
\setboolean{draftmargin}{false}

\IfFileExists{draft_control.tex}{%
\message{Draft control file exists.}%
\input{draft_control.tex}%
}{% 
\message{ WARNING: draft_control.tex not found.}%
\newcommand{\svnVersion}{???}%
}


\ifthenelse{ \boolean{draftmargin} }
        {
                \margintext{Rev: {\svnVersion}\hspace{1em}Built: {\the\year-\pt@twodigit\month-\pt@twodigit\day} {\printtime}}
        }
        {}

\makeatother



==> layout_commands.tex <==
\usepackage{ifthen}
\usepackage{amsmath}
\usepackage{amsthm}

\makeatletter

\newcommand{\titlefamily}{}
\newcommand{\thmfamily}{}
\newcommand{\sectitlefnt}{}
\newcommand{\subsectitlefnt}{}
\newcommand{\ps@footnumber}{}

\newcommand{\authname}[1]{#1}
\newcommand{\authaddress}[1]{#1}

%% Typesetting equations
\renewcommand{\theequation}{\arabic{section}.\arabic{equation}}
\numberwithin{equation}{section}

\newcommand{\fillbox}{\hspace*{\fill}\ensuremath{\Box}}
\renewcommand{\qedsymbol}{\fillbox}

\ifthenelse{\isundefined{\nofancylayout}}
{%
  \renewcommand{\titlefamily}{\sffamily}%
  \renewcommand{\thmfamily}{\sffamily}%
  \renewcommand{\sectitlefnt}{\titlefamily\bfseries\Large}%
  \renewcommand{\subsectitlefnt}{\titlefamily\bfseries}%
  % 
  %% Paper size and margins
  % \usepackage[shiftmargins]{vmargin}
  % \setpapersize{A4}%
  % \setmarginsrb{35mm}{25mm}{30mm}{25mm}{0mm}{0mm}{10mm}{3\baselineskip}%
  %
  \usepackage{calc}
  \usepackage[totalwidth=136mm,totalheight=213mm,vmarginratio=4:5,footskip=3\baselineskip,hcentering]{geometry}
  
  %% Typesetting the titles
  \renewcommand{\section}{\@startsection%
    {section}%
    {1}%
    {0mm}%
    {-\baselineskip}%
    {\baselineskip}%
    {\sectitlefnt}}%
  \renewcommand{\subsection}{\@startsection
    {subsection}%
    {2}%
    {0mm}%
    {-\baselineskip}%
    {0.5\baselineskip}%
    {\subsectitlefnt}}%
  \renewcommand{\ps@footnumber}{%
    \renewcommand{\@oddhead}{}%
    \renewcommand{\@evenhead}{}%
    \renewcommand{\@oddfoot}{\hfill{\thepage}}%
    \renewcommand{\@evenfoot}{{\thepage}\hfill}}

  % 
  %% Typesetting Paragraphs
  \setlength{\parskip}{1ex plus .5ex minus 0ex}
  \setlength{\parindent}{0em}
  % 
  %% Typesetting Theorems
  \newtheoremstyle{my_plain}%
  {\parskip}% above skip
  {\parskip}% below skip
  {\normalfont\itshape}% body font
  {}% indent
  {\normalfont\thmfamily\bfseries}% head font
  {.}% headpunct
  { }% headspace
  {}% custom-head-spec
  
  \newtheoremstyle{my_remark}%
  {\parskip}% aboveskip
  {\parskip}% belowskip
  {\normalfont}% bodyfont
  {}% indent
  {\normalfont\thmfamily\bfseries}% headfont
  {.}% headpunct
  { }% headspace
  {}% custom-head-spec
  
  {
    \theoremstyle{my_plain}
    \newtheorem{theorem}{Theorem}[section]
    \newtheorem{proposition}[theorem]{Proposition}
    \newtheorem{corollary}[theorem]{Corollary}
    \newtheorem{lemma}[theorem]{Lemma}
    \newtheorem{definition}[theorem]{Definition}
  }
  
  {
    \theoremstyle{my_remark}
    \newtheorem{remark}[theorem]{Remark}
  }

  \renewcommand{\authname}[1]{\titlefamily #1\hspace*{0pt}\\}
  \renewcommand{\authaddress}[1]{\begin{minipage}{.8\linewidth}\centering\titlefamily\footnotesize
      #1\hspace*{0pt}\end{minipage}\\[1ex]}
}{%
  \newtheorem{theorem}{Theorem}[section]%
  \newtheorem{proposition}[theorem]{Proposition}%
  \newtheorem{corollary}[theorem]{Corollary}%
  \newtheorem{lemma}[theorem]{Lemma}%
  \newtheorem{definition}[theorem]{Definition}%
  \theoremstyle{remark}%
  \newtheorem{remark}[theorem]{Remark}%
}

\newenvironment{abst}{\begin{quote}\small\thmfamily\bfseries
    Abstract. \normalfont\small}{\end{quote}}

\def\blfootnote{\xdef\@thefnmark{}\@footnotetext}
\makeatother


==> riviere.tex <==
\section{Conservation laws a la Riviere}
\label{sec:riviere}
Here we reproduce the conservation laws for Willmore surfaces in $\mathbb{R}^3$ which are needed in order to conclude the analyticity of Willmore surfaces. 

We let $f:\Sigma\rightarrow \mathbb{R}^3$ a smooth immersion and we let the Gauss map be defined by
\[
x\rightarrow n(x).
\]
Moreover we have the second fundamental form
\[
A=-\langle \nabla f,\nabla n\rangle n
\]
and the mean curvature vector
\[
\bf{H}\rm =\frac12 trA=Hn.
\]

Now the Euler Lagrange equation we consider is
\begin{align}
\Delta_g H+2H(H^2-K)=0, \label{EL}
\end{align}
where $g$ is the induced metric and $K$ is the Gaussian curvature.

In the following we also assume that we have a conformal parametrization
\[
\Phi:B_1(0)\subset \mathbb{R}^2 \rightarrow \mathbb{R}^3
\]
of $\Sigma$. hence we know that $\Sigma=\Phi(B_1(0))$.

We let $\lambda$ be defined by
\[
e^\lambda=|\Phi_x|=|\Phi_y|
\]
and we let $e_1,e_1$ be the orthonormal basis of $T_\Phi \Sigma$, given by
\[
e_1=e^{-\lambda}\Phi_x, \ \ \ e_2=e^{-\lambda}\Phi_y.
\]
Next we note that in this situation we have $A_{ij}=h_{ij}n$, where
\[
h_{ij}=-e^{-\lambda}\langle e_j, n_{x_i} \rangle=h_{ji}.
\]
Moreover we have that
\[
\Delta \Phi=2e^{2\lambda} \bf{H}\rm.
\]


Later on we also need the following Lemma, where here and in the following we use the conventions
\begin{align*}
e_1\wedge e_2=& n\\
n\wedge e_1=&e_2\ \ \ \text{and}\\
e_2 \wedge n=& e_1.
\end{align*}

\begin{lemma}\label{gauss}
With the above conventiones we have
\begin{align}
2Kn=-e^{-2\lambda} (\nabla n\wedge \nabla^\perp n),\label{gauss1}
\end{align}
where $\nabla^\perp=(-\partial_y,\partial_x)$.
\end{lemma}
\begin{proof}
We know that
\[
K=h_{11}h_{22}-h_{12}^2
\]
and hence, by inserting the above formula for $h_{ij}$ we get
\begin{align*}
K=& e^{-2\lambda} (\langle e_1,n_x\rangle \langle e_2,n_y\rangle-\langle e_1,n_y\rangle \langle e_2,n_x\rangle)\\
=& e^{-2\lambda}(n_x^1n_y^2-n_y^1n_x^2).
\end{align*}
Since $\nabla n=\nabla n^1 e_1+\nabla n^2 e_2$ we moreover have 
\begin{align*}
\nabla n \wedge \nabla^\perp n=& (\nabla n^1 \cdot \nabla^\perp n^2-\nabla n^2 \cdot \nabla^\perp n^1)n\\
=& (-n_x^1n_y^2+n^1_yn_x^2-n_y^2n_x^1+n_x^2n_y^1)n\\
=& -2(n_x^1n_y^2-n^1_yn_x^2)n\\
=& -2 e^{2\lambda} Kn.
\end{align*}
\end{proof}

The next lemma contains another important calculation.

\begin{lemma}\label{help}
Using the notations from above we have
\begin{align}
-2H\nabla \Phi=\nabla n+n\wedge \nabla^\perp n. \label{help1}
\end{align}
\end{lemma}
\begin{proof}
We calculate
\begin{align*}
n\wedge \nabla^\perp n=& n\wedge (\nabla^\perp n^1 e_1+\nabla^\perp n^2 e_2)\\
=& \nabla^\perp n^1 e_2 -\nabla^\perp n^2 e_1.
\end{align*}
Using the symmetry of $h_{ij}$ ($n_x^2=n_y^1$) we moreover have
\begin{align}
n\wedge \nabla^\perp n=& \left( \begin{array}{c}
-n_y^1 \\
n_x^1\end{array} \right) e_2-\left( \begin{array}{c}
-n_y^2  \\
n_x^2\end{array} \right)e_1 \nonumber \\
=& -\nabla n^2 e_2 -\nabla n^1 e_1 + (n_x^1+n_y^2)\Big(\left( \begin{array}{c}
1 \\
0\end{array} \right)e_1 + \left( \begin{array}{c}
0 \\
1\end{array} \right)e_2\Big)\nonumber \\
=&-\nabla n-e^\lambda(h_{11}+h_{22})e^{-\lambda} \nabla \Phi \nonumber \\
=&-\nabla n -2H\nabla \Phi.\label{nwedgen}
\end{align}
\end{proof}

Taking the divergence of equation \eqref{help1} yields 
\[
-2H\Delta \Phi-2\nabla H \nabla \Phi=\text{div} (\nabla n+n\wedge \nabla^\perp n).
\]
Multiplying this equation by $H$ and using \eqref{help1} once more gives
\begin{align*}
-2H^2 \Delta \Phi+\nabla H (\nabla n+n\wedge \nabla^\perp n)=H \text{div} (\nabla n+n\wedge \nabla^\perp n).
\end{align*}
Now we also know that
\[
\Delta \Phi=2e^{2\lambda} Hn
\]
and therefore 
\[
-2H^2 \Delta \Phi=-4e^{2\lambda} H^3n=2\Delta H n-4e^{2\lambda}HKn,
\]
where we used \eqref{EL} in the last equality. Combining these equations and using \eqref{gauss1} we therefore get
\begin{align}
2\Delta H n=&H \Delta n-H(\nabla n \wedge \nabla^\perp n) -\nabla H (\nabla n+n\wedge \nabla^\perp n). \label{help2}
\end{align}
Next we have the main theorem of this section.
\begin{theorem}\label{cons}
Let $\Sigma$ be a conformally parametrized Willmore surface as above. Then we have
\begin{align}
\text{div}\Big(H\nabla n-2\nabla H n-H n\wedge \nabla^\perp n\Big)=0.\label{cons1}
\end{align}
\end{theorem}
\begin{proof}
We calculate
\begin{align*}
\text{div}\Big(&H\nabla n-2\nabla H n-H n\wedge \nabla^\perp n\Big)\\
&= H\Delta n-\nabla H\nabla n-2\Delta H n-\nabla Hn\wedge \nabla^\perp n-H\nabla n\wedge \nabla^\perp n
\end{align*}
and by using \eqref{help2} we see that all terms on the right hand side cancel each other.
\end{proof}

In the following we derive even more conservation laws.

Since $B_1(0)$ is contractible we can apply Poincare's Lemma and we get from \eqref{cons1} that there exists a map $L:B_1(0)\rightarrow \mathbb{R}^3$ such that
\[
\nabla^\perp L =H\nabla n-2\nabla H n-H n\wedge \nabla^\perp n.
\]
We have the following theorem.
\begin{theorem}\label{cons2}
We have
\begin{align}
\nabla^\perp L \cdot \nabla \Phi=& 0\ \ \ \text{and} \label{cons2a}\\
\nabla \Phi \wedge \nabla^\perp L=& 2\nabla^\perp H \nabla \Phi. \label{cons2b}
\end{align}
\end{theorem}
\begin{proof}
By \eqref{nwedgen} we know that
\begin{align*}
-n\wedge \nabla^\perp n=\nabla n+2H\nabla \Phi.
\end{align*}
Taking the scalar product of this equation with $\nabla \Phi$ we get
\begin{align*}
-n\wedge \nabla^\perp n\cdot \nabla \Phi= \nabla n\cdot \nabla \Phi +2H \nabla \Phi \cdot \nabla \Phi.
\end{align*}
Now by definition
\[
H=\frac12(h_{11}+h_{22})=-\frac{e^{-2\lambda}}{2}\nabla n \cdot \nabla \Phi .
\]
Moreover
\[
\nabla \Phi \cdot \nabla \Phi=2e^{2\lambda}.
\]
Inserting these two facts into the above equation we get
\begin{align*}
-n\wedge \nabla^\perp n\cdot \nabla \Phi= \nabla n\cdot \nabla \Phi -2\nabla n\cdot \nabla \Phi=-\nabla n\cdot \nabla \Phi.
\end{align*}
Hence we conclude
\begin{align*}
\nabla^\perp L \cdot \nabla \Phi=& H(\nabla n-n\wedge \nabla^\perp n)\cdot \nabla \Phi-2\nabla H n\cdot \nabla \Phi\\
=&0,
\end{align*}
since $n\cdot \nabla \Phi=0$. This finishes the proof of \eqref{cons2a}.

Using again \eqref{nwedgen} we have
\[
\nabla \Phi \wedge (n\wedge \nabla^\perp n)= -\nabla \Phi \wedge \nabla n.
\]
Since $h_{ij}=h_{ji}$ we get
\begin{align*}
\nabla \Phi \wedge \nabla n=& \partial_x \Phi \wedge \partial_x n+\partial_y \Phi \wedge \partial_y n\\
=&e^\lambda( e_1 \wedge \partial_x n+e_2\wedge \partial_y n)\\
=&e^\lambda (\langle \partial_x n, e_2 \rangle -\langle \partial_y n, e_1 \rangle)n\\
=&  e^{2\lambda}(-h_{12}+h_{21})n=0.
\end{align*}
Hence this gives
\begin{align*}
H\nabla \Phi \wedge \nabla n-H\nabla \Phi \wedge( n\wedge \nabla^\perp n)=& 2H\nabla \Phi \wedge \nabla n\\
=&0. 
\end{align*}
Therefore it remains to show that
\[
-2\nabla H \nabla \Phi \wedge n=2 \nabla^\perp H  \nabla \Phi.
\]
This can be seen as follows
\begin{align}
\nabla \Phi \wedge n= e^\lambda \left( \begin{array}{c}
e_1\wedge n \\
e_2 \wedge n\end{array} \right)=e^\lambda \left( \begin{array}{c}
-e_2 \\
e_1 \end{array} \right)=\nabla^\perp \Phi.\label{wedgephi}
\end{align}
Moreover we have 
\[
\nabla H\nabla^\perp \Phi=-\nabla^\perp H  \nabla \Phi
\]
and this finishes the proof of \eqref{cons2b} and hence the theorem.
\end{proof}

Next we let (using Poinare's Lemma and theorem \ref{cons2})
\begin{align*}
\nabla S=& L\nabla \Phi\ \ \ \text{and}\\
\nabla R=&\nabla \Phi \wedge L-2H\nabla \Phi
\end{align*}
and we have
\begin{theorem}\label{rs}
We have
\begin{align}
\nabla^\perp R=\nabla S n+\nabla R\wedge n\label{rs1}
\end{align}
and therefore
\begin{align}
\Delta R= -\nabla S \nabla^\perp n-\nabla R \wedge \nabla^\perp n.\label{rs2}
\end{align}
\end{theorem}
\begin{proof}
Our goal is to calculate $\nabla R\wedge n$. In order to do this we note that
\[
(\nabla \Phi \wedge L^T)\wedge n = 0,
\]
where here $L^T=\langle L,e_1\rangle e_1+\langle L,e_2\rangle e_2$. Hence we have
\begin{align*}
 \nabla R\wedge n=& \langle L,n\rangle (\nabla \Phi \wedge n)\wedge n-2H\nabla \Phi\wedge n\\
=& \nabla^\perp \Phi \wedge (\langle L,n\rangle n)-2H\nabla^\perp \Phi\\
=& \nabla^\perp R-\nabla^\perp \Phi \wedge L^T,
\end{align*}
where we used \eqref{wedgephi} in the second step. Next we note that
\begin{align*}
\nabla^\perp \Phi \wedge L^T=& e^\lambda \left( \begin{array}{c}
-e_2\wedge \langle L,e_1\rangle e_1+\langle L,e_2\rangle e_2 \\
e_1 \wedge \langle L,e_1\rangle e_1+\langle L,e_2\rangle e_2\end{array} \right)\\
=& e^\lambda\left( \begin{array}{c}
 \langle L,e_1\rangle \\
\langle L,e_2\rangle\end{array} \right)n\\
=& L\nabla \Phi n =\nabla S n.
\end{align*}
Combining all these facts finishes the proof of the first statement. The second one is an easy consequence of the first one, since $\Delta=-\nabla^\perp( \nabla^\perp)$ and $\nabla^\perp (\nabla)=0$.
\end{proof}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "master"
%%% ispell-local-dictionary: "en_US"
%%% End: 

